NeuralMPS: Non-Lambertian Multispectral Photometric Stereo via Spectral Reflectance Decomposition

Multispectral photometric stereo(MPS) aims at recovering the surface normal of a scene from a single-shot multispectral image captured under multispectral illuminations. Existing MPS methods adopt the Lambertian reflectance model to make the problem tractable, but it greatly limits their application to real-world surfaces. In this paper, we propose a deep neural network named NeuralMPS to solve the MPS problem under general non-Lambertian spectral reflectances. Specifically, we present a spectral reflectance decomposition(SRD) model to disentangle the spectral reflectance into geometric components and spectral components. With this decomposition, we show that the MPS problem for surfaces with a uniform material is equivalent to the conventional photometric stereo(CPS) with unknown light intensities. In this way, NeuralMPS reduces the difficulty of the non-Lambertian MPS problem by leveraging the well-studied non-Lambertian CPS methods. Experiments on both synthetic and real-world scenes demonstrate the effectiveness of our method.

==> images/reflectance_decomp/ref_demp.tex <==
	\resizebox{0.5\textwidth}{!}{
		\Large
		\begin{tabular}{cc@{}@{}c|c@{}@{}c@{}@{}c}
			\raisebox{2em}{\makebox[0.05\textwidth][c]{\makecell[c]{Paper \\ blue}}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/reflectance_decomp/paper_blue_rendering_1.jpg}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/fig3/paper_blue_gt.pdf}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/fig3/paper_blue_light.pdf}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/fig3/paper_blue_geo.pdf}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/fig3/paper_blue_rec.pdf}}\\
			\raisebox{2em}{\makebox[0.05\textwidth][c]{\makecell[c]{ilm \\ l3 \\ 37 \\ matte}}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/reflectance_decomp/paper_red_rendering_1.jpg}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/fig3/ilm_l3_37_matte_gt.pdf}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/fig3/ilm_l3_37_matte_light.pdf}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/fig3/ilm_l3_37_matte_geo.pdf}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/fig3/ilm_l3_37_matte_rec.pdf}}					
	\end{tabular}
	}

==> table/img_formation_comp.tex <==
	\resizebox{0.5\textwidth}{!}{
		\begin{tabular}{cc}
		\toprule
		Task & Reflectance definition \\
		\midrule
		CPS, non-Lambertian & $r_i = R(\V{l}_i, \V{v}, \V{n})$ 
	 	\\
		[-0.5em]
		\\
		 MPS, Lambertion & \hbox{$r_{i}= \int_{\lambda \in \Omega_i} E_i(\lambda)R(\lambda) S_i(\lambda) d\lambda$}
		 \\
		 [-0.5em]
		 \\
		 MPS, non-Lambertian& \hbox{$r_{i}= \int_{\lambda \in \Omega_i} E_i(\lambda)R(\V{l}_i, \V{v}, \V{n}, \lambda) S_i(\lambda) d\lambda$} \\
		 \bottomrule
		\end{tabular}
	}

==> table/method_compare.tex <==
\resizebox{0.48\textwidth}{!}{
	\begin{threeparttable}
		\begin{tabular}{ccc}
			\toprule
			&Lambertian & Non-lambertian \\
			\midrule
			Time-multiplexing &\cite{silver1980determining, woodham1980ps} & \cite{wu2010robust}\\
			Spectral-multiplexing & \cite{kontsevich1994, drew1994closed, ozawa2018single, chakrabarti2016single, fyffe2011single, miyazaki2019color, anderson2011augmenting, anderson2011color, guo2021mps} & \cite{antensteiner2019single, ju2018demultiplexing, ju2020mps, ju2020dual}	\\
			\bottomrule	
		\end{tabular}
	\end{threeparttable}
		}
